Direct Simultaneous Translation Activation for Large Audio-Language Models

Simultaneous speech-to-text translation (Simul-S2TT) aims to translate speech into target text in real time, outputting translations while receiving source speech input, rather than waiting for the entire utterance to be spoken. Simul-S2TT research often modifies model architectures to implement read-write strategies. However, with the rise of large audio-language models (LALMs), a key challenge is how to directly activate Simul-S2TT capabilities in base models without additional architectural changes. In this paper, we introduce {\bf Simul}taneous {\bf S}elf-{\bf A}ugmentation ({\bf SimulSA}), a strategy that utilizes LALMs' inherent capabilities to obtain simultaneous data by randomly truncating speech and constructing partially aligned translation. By incorporating them into offline SFT data, SimulSA effectively bridges the distribution gap between offline translation during pretraining and simultaneous translation during inference. Experimental results demonstrate that augmenting only about {\bf 1\%} of the simultaneous data, compared to the full offline SFT data, can significantly activate LALMs' Simul-S2TT capabilities without modifications to model architecture or decoding strategy.

==> 6-related-work.tex <==
% \section{Related Work}
% \subsection{Large Audio-Language Model}
% The success of large language models~\cite{brown2020languagemodelsfewshotlearners, zhao2025surveylargelanguagemodels,yang2024qwen2} in text-based applications has spurred growing interest in extending these models to speech-related tasks. Recent works~\cite{tang2024salmonn,chu2023qwen,chu2024qwen2,ghosh2024gama,gong2024listenthinkunderstand} typically leverage architectures that couple an audio encoder—such as Whisper~\cite{radford2022robustspeechrecognitionlargescale} or Conformer~\cite{gulati2020conformerconvolutionaugmentedtransformerspeech}—with pretrained LLMs, like LLaMA~\cite{Touvron2023LLaMAOA}, Vicuna~\cite{vicuna2023}, or Qwen~\cite{bai2023qwentechnicalreport,yang2024qwen2technicalreport,yang2024qwen2}. 
% To address the mismatch in sequence lengths between speech and text modalities, some studies~\cite{Wu2023OnDA,tang2024salmonn} introduce length adapters that compress speech representations following the encoder. While most methods rely on a fixed set of prompts or special tokens to support multitasking, others~\cite{chu2024qwen2} explore instruction tuning and direct preference optimization~\cite{Rafailov2023DirectPO} to better handle natural language instructions and align with human preferences. Despite these advances, dedicated research on simultaneous speech-to-text translation using large audio-language model (LALM) remains sparse.


% \subsection{Simultaneous Speech-to-Text Translation}
% Simultaneous Speech-to-Text Translation (Simul-S2TT), or real-time speech translation, faces the inherent challenge of processing streaming, fragmented audio input to produce accurate and low-latency translations.
% Traditional methods like the wait-k strategy~\cite{ma-etal-2019-stacl}, balance translation quality and latency by introducing a fixed delay before generating translation. Monotonic Infinite Lookback attention~\cite{arivazhagan-etal-2019-monotonic} further balances these factors in text-based settings. 
% However, unlike text, speech presents a continuous signal, making it challenging to establish semantic boundaries at intermediate points of the audio stream.
% Recent advances~\cite{papi-etal-2024-streamatt} explore dynamic utilization of audio and text context to aid translation decisions. Other approaches~\cite{deng-woodland-2024-label, yu-etal-2024-self} introduce extra networks to learn adaptive read/write policies at each decoding step, albeit at the cost of architectural complexity and higher computational overhead.

% Emerging studies are beginning to leverage LALMs for Simul-S2TT. ~\citep{cheng2024achievinghumanparityendtoend} employs LLMs to segment transcripts into semantic chunks, and then translate to construct aligned streaming audio-translation pairs. Nonetheless, research in this direction is still limited. In this work, we propose leveraging LALMs for Simul-S2TT without modifying the original model architecture or incurring additional inference costs. Our approach flexibly supports variable translation intervals, enabling scalable and efficient simultaneous speech-to-text translation in practical scenarios.

\section{Related Work}

\subsection{Large Audio-Language Models}
Large language models (LLMs) have been highly successful in text tasks~\cite{brown2020languagemodelsfewshotlearners, zhao2025surveylargelanguagemodels,yang2024qwen2}. This has motivated their application to speech tasks. Recent studies~\cite{tang2024salmonn,chu2023qwen,chu2024qwen2,ghosh2024gama,gong2024listenthinkunderstand} combine audio encoders like Whisper~\cite{radford2022robustspeechrecognitionlargescale} or Conformer~\cite{gulati2020conformerconvolutionaugmentedtransformerspeech} with pretrained LLMs such as LLaMA~\cite{Touvron2023LLaMAOA}, Vicuna~\cite{vicuna2023}, or Qwen~\cite{bai2023qwentechnicalreport,yang2024qwen2technicalreport,yang2024qwen2}. To match speech and text lengths, some use length adapters~\cite{Wu2023OnDA,tang2024salmonn}. While many methods use fixed prompts for multiple tasks, others~\cite{chu2024qwen2} use instruction tuning to better follow natural language commands. However, using large audio-language models for real-time speech translation is still under-explored.

\subsection{Simultaneous Speech-to-Text Translation}
Simultaneous Speech-to-Text Translation (Simul-S2TT) translates speech in real-time, requiring quick and accurate processing of continuous audio. Traditional methods like the wait-k strategy~\cite{ma-etal-2019-stacl} add a fixed delay to balance speed and quality. Monotonic Infinite Lookback attention~\cite{arivazhagan-etal-2019-monotonic} also aims to achieve this balance. Unlike text, speech lacks clear breaks, making real-time translation harder.
Recent approaches~\cite{papi-etal-2024-streamatt} use both audio and text context to improve translations. Other methods~\cite{deng-woodland-2024-label, yu-etal-2024-self} add networks to decide when to read more audio or write translations, but these add complexity. Some new studies use large audio-language models for Simul-S2TT. For example,~\citep{cheng2024achievinghumanparityendtoend} segments transcripts into meaningful parts for translation. However, this area is still new. In this work, we use large audio-language models for real-time translation without changing their structure or adding extra steps. Our method allows flexible timing, making real-time translation more efficient and practical.
